Active Velocity Estimation using Light Curtains via Self-Supervised Multi-Armed Bandits

To navigate in an environment safely and autonomously, robots must accurately estimate where obstacles are and how they move. Instead of using expensive traditional 3D sensors, we explore the use of a much cheaper, faster, and higher resolution alternative: programmable light curtains. Light curtains are a controllable depth sensor that sense only along a surface that the user selects. We adapt a probabilistic method based on particle filters and occupancy grids to explicitly estimate the position and velocity of 3D points in the scene using partial measurements made by light curtains. The central challenge is to decide where to place the light curtain to accurately perform this task. We propose multiple curtain placement strategies guided by maximizing information gain and verifying predicted object locations. Then, we combine these strategies using an online learning framework. We propose a novel self-supervised reward function that evaluates the accuracy of current velocity estimates using future light curtain placements. We use a multi-armed bandit framework to intelligently switch between placement policies in real time, outperforming fixed policies. We develop a full-stack navigation system that uses position and velocity estimates from light curtains for downstream tasks such as localization, mapping, path-planning, and obstacle avoidance. This work paves the way for controllable light curtains to accurately, efficiently, and purposefully perceive and navigate complex and dynamic environments. Project website: https://siddancha.github.io/projects/active-velocity-estimation/

==> sections/evaluation-metric.tex <==
\section{Evaluation metrics}
\label{sec:evaluation-metric}
\dave{Note - I moved this section from where it was previously in the middle of the methods section; since this section is about evaluation it should go in the results section.}
\sid{I agree that it usually makes sense to discuss evaluation metrics after the methods section. I think this particular paper is an exception. The reason is that our self-supervised reward is a modified version of the forecasted occupancy metric. I think it is helpful for the reader to first understand \textit{why} forecasted occupancy is a useful metric to begin with, before we explain \textit{how} we are able to compute it in a self-supervised way for multi-armed bandits in the absence of ground-truth. If we delay this to the experiments section, I find myself having to repeat the same arguments in Sec. 7. Therefore, I have moved this section back here for now. If you have a better flow in mind I'm happy to move this to the experiments section.}\dave{Yes I do have a better flow in mind - see the organization that I used when I moved things around.  The current organization is much worse and is likely to get your paper rejected. I am happy to discuss this further over Zoom.}

We wish to evaluate the accuracy of both occupancy and velocity estimates. A metric that simultaneously captures both accuracies is \textit{forecasted occupancy}~\cite{mahjourian2022occupancy,waymo2022challenge}.
The current occupancy and velocity at timestep $t$ is evaluated by computing the occupancy at a future timestep $t + \Delta t$. To do so, the current velocity is used to forecast the current occupancy by an interval $\Delta t$ %We evaluate the current dynamic occupancy grid by forecasting it 
using a motion update step (see Sec.~\ref{sec:dynamic-occupancy-grids}, \app~\ref{app:motion-update-step}).
%, and compare the forecasted grid with ground truth occupancy.
The forecasted occupancy will be accurate if both the current occupancy and current velocities are accurate. This metric is particularly relevant for obstacle avoidance where future occupancy of obstacles is required to plan collision-free paths.

The accuracy of forecasted occupancy is computed by comparing it against ground truth occupancy at $t + \Delta t$.
% \dave{But we don't know the ground-truth occupancy - please comment on how the evaluation metric is actually computed.}
Ground truth occupancy is available for all grid cells in simulated environments. In real-world environments, true occupancy can only be measured for a subset of cells by the light curtain; in this case, we use a ``self-supervised'' version of this metric described in Sec.~\ref{sec:mab}.
% We evaluate the current dynamic occupancy grid by forecasting it using a motion update step (see Sec.~\ref{sec:dynamic-occupancy-grids}, \app~\ref{app:motion-update-step}), and compare the forecasted grid with ground truth occupancy.
We follow prior works~\cite{hornung2013octomap,meyer2012occupancy,tatarchenko2017octree} that treat the evaluation of occupancy as a classification problem and compute several metrics: (1) classification accuracy~\cite{hornung2013octomap,meyer2012occupancy}, (2) precision, (3) recall, (4) \fone-score and (5) the IoU~\cite{tatarchenko2017octree} between the predicted and ground truth occupancy masks. For more details on these metrics, please see \app~\ref{app:evaluation-metric}.
% \dave{Maybe add a note connecting this to our self-supervised reward in Sec.~\ref{sec:mab}}
